Neural Re-ranking in Multi-stage Recommender Systems: A Review

As the final stage of the multi-stage recommender system (MRS), re-ranking directly affects user experience and satisfaction by rearranging the input ranking lists, and thereby plays a critical role in MRS. With the advances in deep learning, neural re-ranking has become a trending topic and been widely applied in industrial applications. This review aims at integrating re-ranking algorithms into a broader picture, and paving ways for more comprehensive solutions for future research. For this purpose, we first present a taxonomy of current methods on neural re-ranking. Then we give a description of these methods along with the historic development according to their objectives. The network structure, personalization, and complexity are also discussed and compared. Next, we provide benchmarks of the major neural re-ranking models and quantitatively analyze their re-ranking performance. Finally, the review concludes with a discussion on future prospects of this field. A list of papers discussed in this review, the benchmark datasets, our re-ranking library LibRerank, and detailed parameter settings are publicly available at https://github.com/LibRerank-Community/LibRerank.

==> hide_text.tex <==
% A key technical challenge for re-ranking is modeling the listwise context (cross-item interactions) of how items are influenced by other items placed in the same list. \qjr{not items are influenced, but the probability of being clicked is influenced} \qjr{need to provide a clear definition of re-ranking: listwise scoring? Thus, major challenge is modeling listwise context}

% Therefore, we classify the re-ranking models according to their objectives into accuracy-oriented re-ranking for single objective methods, and diversity-aware or fairness-aware re-ranking for multiple objectives methods.

% Most work assumes that the relevance label of each item is independent to each other, and thus uses observed fixed labels to train the model (which is also known as the probability ranking principle \cite{robertson1977probability})
% According to the main objective of re-ranking, we classify the existing work into accuracy-oriented re-ranking, diversity-oriented re-ranking, and fairness-oriented re-ranking, as summarized in Figure \ref{fig:orgchart}. The accuracy-oriented re-ranking is further grouped into initial list modeling, and re-ranked list modeling, where the former directly models the listwise context of the input initial list, and the latter focuses on the permutated re-ranked lists. According to the organization of Figure \ref{fig:orgchart}, we observe the following three development observations: (i) compared to the purely accuracy-oriented methods, (ii) researches are developing from initial list modeling to re-ranked list modeling. (iii) more studies concentrate on personalized re-ranking. Moreover, we notice that there is a new trend of evolving from single list re-ranking to integrated re-ranking with multiple lists (discussed in Section \ref{sect:int}). \ruiming{is this part included in figure 2?} 

% \fei{Adding come citations here might be more convincing and helpful.}
% in the upper right corner



% \subsection{Development Trends}
%Practical recommendation applications are restrained by computational limits as the numbers of users and items grow into billions. Therefore, MRS become a natural solution by splitting the recommendation task into multiple steps -- each step narrows down the relevant items with a slower but more accurate ranker \cite{hron2021component}, to guarantee low response latency.
% \qjr{"listwise context" and "hundreds" should have some relations?}

% \qjr{better give an example of the cross-item interactions and put it in section 1}

% \qjr{$\arg\min_{\phi} \sum_{R,Y}$, where is $u$, better use $R_u, Y_u$}
% \qjr{emphasize the difference w.r.t. pointwise scoring function here}


%  \qjr{more specific, xxx in section xxx}
% \qjr{where is the ``neural" part?}

% Other than different structures adopted, another important factor in modeling the listwise context is to determine whether to model the listwise context in the \textit{initial ranking list} \cite{dlcm,prm} or \textit{the reranked list} \cite{gsf,egrerank}. Below we describe various attempts with their advantages and disadvantages for initial list modeling and re-ranked list modeling. \ruiming{personalization is an important factor as in Figure 2, but it is not in the text.}
% The listwise context provides strong signals for items' relevance estimated by ranking models.  
% Towards optimizing the accuracy, one of the key challenges is the modeling of the listwise context. Several techniques have been explored to build such cross-item dependencies and correlations among candidate items, including the recurrent listwise modeling (RNN) \cite{dlcm}, the attentive listwise modeling (self-attention) \cite{prm}, and the graph neural networks (GNN) \cite{irgpr}, 

% A typical architecture of the re-ranking model for initial list modeling can be outlined as in Figure \ref{fig:flowchart}(a), which firstly embeds user and item features into low-dimensional dense vectors, and then extracts cross-item interactions by the listwise context modeling on the initial list, followed by feed-forward networks to generate the re-ranking scores. The initial lists provide strong signals for items' relevance estimated by ranking models.  
% Several existing studies have shown the effectiveness of modeling dependencies among initial lists \cite{dlcm,prm,setrank,feng2021revisit}. 
% estimate re-ranking scores from the initial list, instead of the re-ranked list. The re-ranking operation (sorting the items greedily with the estimated re-ranking scores) changes the context of each item from the initial list to the re-ranked list, while listwise context directly affects the final recommendation quality. In the next section, we will focus on modeling the re-ranked lists.
% which may result in imprecise estimation under new permutations

% Followup work has focused on






% \subsection{Relation with the Ranking Models}

% follow the evaluator-generator paradigm and propose the SEG model. The evaluator is trained to measure the expected utility considering cross-item correlations via multiple network structures, and the generator using the heuristic search or reinforcement learning is devised to generate potential high-quality permutations, from which the evaluator selects the best permutation and displays to the user. They also find that the predictions from the evaluator are positively correlated with the results of the online A/B test, which empirically verifies the usefulness of an evaluator.
% A series of follow-up studies adopt the evaluator-generator paradigm. 

% CDIA is composed of a listwise evaluator and the generator is trained by the temporal difference (TD) method under the supervision of the evaluator. \fei{need citation}
% \citet{gcr} also design the evaluator and generator with reinforcement learning. 
% , and uses Bi-LSTM as the listwise evaluator to capture long-short term correlation within the permutation. 
% GRN \cite{grn} further proposes a generator with RNN, self-attention, and the pointer network to select the next item step by step. 

% \citet{gsf} present an early effort on modeling re-ranked permutations. 
% point out the sensitivity issue to the input order in existing re-ranking models for initial list modeling, and 

% \qjr{enumerating is not enough, pls give some more analysis and explanations: how to get evaluators? Why not directly use the evaluators?}

% ;, showing that apart from forward cross-item dependencies, the backward dependencies also provide critical information for re-ranking, which is consistent with users' comparison behaviors of reverse examination to compare items in the same list \cite{ccm}. 
% % \qjr{with users' reverse comparison behaviors}

% \qjr{give the citation of the pairwise and listwise loss used in re-ranking models, not the original papers of the losses}

% , compared with the pairwise or pointwise losses

% \qjr{what about the latter way?}
% \xx{Should we reflect both types of personalization in the Table 1? As personalizetion by input data can be easily generalized to all models} 
% \xx{It should be noted that the complexity in the table is at the inference stage.}
% \qjr{sounds like it is $\mathcal{O}(1)$.}


% . DSSA jointly estimates the relevance and the diversity given the candidate items, and uses a weighted combination of the two to produce the next item.

% The line of work mainly seeks to enhance diversity and fairness in re-ranking stage for recommender systems. 
% From the view of multi-stakeholder system \cite{liu2019personalized}, the key differences lie in the concerns being addressed and the way in which success is measured. 
% Diversity is usually user-centric and aims to cover diverse user intents, while fairness mostly measures the outcome for under-represented item providers.

% \fei{The statement here may be inaccurate. Fairness can also be measured on items or users, e.g. job recommendation in LinkedIn, reciprocal recommendation in dating platform, or poor results on users with few behaviors (User-oriented Fairness in Recommendation)}
% Alternatively, there are recommendation scenarios that accuracy is not the only objective. Diversity of the re-ranking results is another important measurement, especially for scenarios like news recommendation where obtaining new information is desired. 
% \ruiming{different granularity?} 
% \ruiming{a loss function considering both accuracy and diversity?}
% How to delicately manage the tradeoff between relevance and diversity is a key challenge for diversity-aware re-ranking. 
%  Reinforcement learning is also involved in diversity-aware re-ranking to help the sequential item selection.
% \ruiming{what is the key relationship or difference between diversity and fairness reranking?}
% to re-rank items in different forms of texts, images, or videos.
% An example is shown in Figure \ref{fig:int}. 
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{imgs/integrat_rerank.pdf}
%     \caption{An integrated re-ranking system.}
%     \label{fig:int}
% \end{figure}
% \ruiming{intergrated, fairness, diversity}

% , including , or ads and organic items \cite{dear}.

% DHANR \cite{dhanr} models cross-item interactions using a hierarchical self-attention structure, where the correlations items are captured by both item-level and source-level. The final re-ranking list is obtained by sorting the items from different sources according to the unified reranking scores. \citet{hrlrec} decompose the integrated re-ranking problem into two sub-tasks -- source selection and item ranking. Therefore, they use hierarchical reinforcement learning (HRL) with a low-level agent as a source selector, and a high-level agent as an item recommender to choose the next item from the selected source. DEAR \cite{dear,ram} learns to interpolate ads and organic items by a deep Q-network. \citet{liao2021cross} also adopts a reinforcement learning solution. They find that extracting cross information between actions and states benefits the integrated re-ranking and propose the CrossDQN model. 

% We conduct benchmarking experiments on two public recommendation datasets, \textbf{Ad}\footnote{https://tianchi.aliyun.com/dataset/dataDetail?dataId=56} and \textbf{PRM Public}\footnote{https://github.com/rank2rec/rerank}. For Ad dataset, items that have been interacted within five minutes are sliced into a list following \cite{grn,prs}. These two datasets contain user and item features with recommendation lists, allowing experimentation with personalized re-ranking. Datasets are downsampled due to the memory limitation, the remained dataset details are summarized in Table \ref{tab:dataset}. Depending on the length of the initial ranking, the maximum length of initial lists (re-ranking size $n$) is set to 10 and 30 for Ad and PRM Public, respectively. These benchmark datasets are also released together with the \texttt{PyR} library. \

% More implementation details including the data processing and the parameter settings are available online\footnote{link here}.

% \subsection{Dataset and Data Processing}
% The positive items are usually much larger than the negative ones, as the user mostly only click one item for each list. To balance the positive and negative samples, all zeros

% We conduct experiments on two public datasets, including E-commerce Re-ranking dataset\footnote{https://github.com/rank2rec/rerank} and Ad dataset\footnote{https://tianchi.aliyun.com/dataset/dataDetail?dataId=56}. 
% \begin{itemize}
%     \item \textbf{PRM Public} contains 743, 720 users, 7, 246, 323 items, and 14, 350, 968 records in the form of reranking lists obtained from a real-world e-commerce RS. Each record is a recommendation list consisting of 3 user profile features, 5 categorical, and 19 dense item features. Since the raw data is very large, we randomly sampled 10\% of the reranking lists in our experiments.
%     \item \textbf{Ad} records 1, 140, 000 users and 26 million ad display or click logs, with 9 user profiles (e.g., id, age, and occupation), 6 item features (e.g., id, campaign, and brand), and user shopping history of seven hundred million records. Following \cite{grn,prs}, we transform records of each user into ranking lists according to the timestamp of the user browsing the advertisement. Items that have been interacted within last five minutes are sliced into a list. 
% \end{itemize}
% After obtaining the processed lists, we slice them in a 4:5:1 ratio for initial ranker training, reranking model training and reranking model testing, respectively. We select a widely adopted state-of-the-art ranking algorithm, LambdaMART \cite{lambdamart}, as the initial ranking, with item embeddings pre-trained by DNN. According to different recommendation scenarios, the maximum length of initial lists is set to 30 and 10 for PRM Public and Ad, respectively.
% We compare several state-of-the-art reranking models, including DLCM, PRM, SetRank, GSF, and MIDNN. To ensure a fair comparison, we fine-tune all models to achieve their best performance.

% \subsection{Quantitative Comparison}

% the pointwise cross-entropy loss (CE) is the most adopted loss due to its simplicity and effectiveness. 
% The pairwise loss BPR loss (BPR) \cite{rendle2012bpr} or the hinge loss (Hinge) \cite{bartlett2008classification} compares two items simultaneously and optimize the relative positions of two items. The listwise loss, Attention Rank loss (AttRank) \cite{dlcm} and the KL loss (KL) \cite{listcvae}, further considers the listwise difference between the predicted scores and the target distribution.
% The listwise losses, though model the cross-item interactions from the loss level, are usually more difficult and expensive to train \cite{guo2020deep}.

%  the generator-evaluator models rely on dense and instant feedback labels for effective training, which are originally provided by a simulation environment in their work. While Ad and PRM Public are extremely sparse. Moreover, 

% \ruiming{counterfactual, multi-objectives}

% \subsubsection{Data Imbalance}
% The training data for re-ranking is mostly imbalanced. Different requests may have different amounts of labeled items, and positive items in the list are much fewer than negative items. Qiu \etal provide a good attempt in addressing the data imbalance issue by proposing a data generation module to augment the training data with variational auto-encoder for re-ranking. 
